Learning to Learn Weight Generation via Local Consistency Diffusion

Diffusion-based algorithms have emerged as promising techniques for weight generation. However, existing solutions are limited by two challenges: generalizability and local target assignment. The former arises from the inherent lack of cross-task transferability in existing single-level optimization methods, limiting the model's performance on new tasks. The latter lies in existing research modeling only global optimal weights, neglecting the supervision signals in local target weights. Moreover, naively assigning local target weights causes local-global inconsistency. To address these issues, we propose Mc-Di, which integrates the diffusion algorithm with meta-learning for better generalizability. Furthermore, we extend the vanilla diffusion into a local consistency diffusion algorithm. Our theory and experiments demonstrate that it can learn from local targets while maintaining consistency with the global optima. We validate Mc-Di's superior accuracy and inference efficiency in tasks that require frequent weight updates, including transfer learning, few-shot learning, domain generalization, and large language model adaptation.

==> sec/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper’s contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: Our Abstract (lines 1–14) clearly identifies the two core challenges (generalizability and local target assignment) and summarizes our three contributions—(1) the Mc-Di framework combining diffusion with meta-learning, (2) the local consistency diffusion algorithm, and (3) convergence improvements via SAM—with detailed presentation in Section 1 and Figure 2.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation, as long as it is clear that these goals are not attainable by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: We explicitly discuss the limitation of relying on a fixed Gaussian inference starting point and outline future work adopting more general trajectory methods (Flow Matching, Trajectory Balance) in Section 5 (“Limitation and future work”).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitations, while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed not to penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: All formal definitions, assumptions, and proofs of Theorems 1–2 (local consistency diffusion and convergence bound) are given in Appendices A–C following the statements in the main text (Section 3).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in the appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: We detail dataset splits, baselines, optimizer settings (learning rates, inner/outer‐loop steps, segment number \(k\), diffusion steps \(T\)), and hardware platform in Section 4.2 and Appendix E, and provide Algorithm 1–2 pseudocode for the weight preparation and meta‐training stages.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, no answer to this question will not be perceived well by the reviewers: making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, the paper should make it clear how to reproduce that algorithm.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution.
    \end{itemize}

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in the supplemental material?
    \item[] Answer: \answerNo{}
    \item[] Justification: No URL or repository for code or processed data is provided in the submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer.
    \end{itemize}

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Training/test details (datasets, Meta-training/Meta-testing splits, learning rates, early‐stopping, segment number \(k\), diffusion steps \(T\)) are described in Section 4.2 and Algorithm 1–2, with further hyperparameter choices documented in Appendix E.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in the appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: All quantitative results are reported as mean ± standard deviation over five independent runs (see Tables 1–5).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: We report use of two NVIDIA A100 GPUs, one Intel Xeon Gold 6348 CPU, and 512 GB RAM; per-experiment GPU‐hour budgets are indicated in Section 4.1–4.2.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers (CPU/GPU), including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
    \end{itemize}

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerNA{}
    \item[] Justification: Our work does not involve human subjects, sensitive data, or dual‐use concerns.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
    \end{itemize}

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}
    \item[] Justification: This foundational method for weight generation has no direct societal applications or risks discussed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
    \end{itemize}

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse?
    \item[] Answer: \answerNA{}
    \item[] Justification: We do not release models or datasets with dual‐use risk.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets used in the paper properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: We cite all works properly.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: We introduce no new datasets or pretrained models beyond our method.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: No human‐subject or crowdsourcing studies are conducted.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether IRB approvals were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: Not applicable—no human subjects research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research?
    \item[] Answer: \answerYes{}
    \item[] Justification: We apply Mc-Di to generate LoRA matrices for RoBERTa-base fine-tuning and report adaptation accuracy and latency in Section 4.2.4.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> sec/rebuttal.tex <==
\setcounter{table}{8}
\setcounter{figure}{8}


% \begin{table*}[t]
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Method} & \textbf{CIFAR-10} & \textbf{CIFAR-100} & \textbf{Omniglot} & \textbf{Mini-ImageNet} \\
% \midrule
% \rowcolor{gray!20} Linear Decay(ours) & 62.07 ± 0.33 & 51.73 ± 0.25 & 97.12 ± 0.23 & 68.10 ± 0.24 \\
% Power-law Decay & 61.70 ± 0.36 & 51.42 ± 0.23 & 96.54 ± 0.25 & 67.69 ± 0.21 \\
% Exponential Decay & 61.57 ± 0.29 & 51.51 ± 0.29 & 96.34 ± 0.27 & 67.56 ± 0.26 \\
% \bottomrule
% \end{tabular}
% \caption{Sensitive study of Lt-Di under different scheduling strategies for $\gamma_i$.}
% \label{tab:schedule_ablation}
% \end{table*}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{lt_di_schedule_ablation.pdf}
    \caption{Sensitive study of Lt-Di under different $\gamma_i$ scheduling strategies.}
    \label{tab:schedule_ablation}
\end{figure}

\begin{table*}[t]
\centering
\begin{tabular}{lccccccc}
\toprule
\textbf{Method} & \textbf{Traffic Sign} & \textbf{MSCOCO} & \textbf{MNIST} & \textbf{CIFAR-100} & \textbf{CIFAR-10} & \textbf{Avg} & \textbf{Latency (ms)} \\
\midrule
REPTILE & 50.32 ± 0.88 & 43.62 ± 1.02 & 72.50 ± 0.88 & 45.60 ± 0.98 & 48.73 ± 0.94 & 52.55 & 26.8 \\
Meta-Baseline & 47.52 ± 0.92 & 41.20 ± 1.04 & 68.47 ± 0.85 & 43.07 ± 0.85 & 46.02 ± 0.90 & 49.26 & 26.2 \\
Meta-Hypernetwork & 55.91 ± 0.91 & 48.47 ± 0.91 & 80.55 ± 0.91 & 50.67 ± 0.91 & 54.14 ± 0.91 & 57.15 & 10.3 \\
GHN3 & 44.22 ± 0.93 & 47.27 ± 1.14 & 76.44 ± 0.91 & 36.38 ± 0.83 & 42.52 ± 1.06 & 49.37 & 30.1 \\
OCD & 52.14 ± 0.90 & 57.74 ± 1.12 & 75.23 ± 0.92 & 47.51 ± 0.91 & 55.54 ± 1.13 & 57.63 & 9.7 \\
Meta-Diff & 57.19 ± 0.94 & 60.01 ± 1.04 & 78.47 ± 0.94 & 55.29 ± 0.89 & 61.38 ± 1.01 & 62.47 & 10.9 \\
\rowcolor{gray!20} Lv-Di (ours) & 56.48 ± 1.02 & 60.58 ± 1.00 & 80.82 ± 0.93 & 55.13 ± 0.93 & 62.93 ± 1.04 & 63.19 & 7.0 \\
\rowcolor{gray!20} Lt-Di (ours) & 58.46 ± 0.99 & 62.70 ± 1.01 & 83.65 ± 0.94 & 57.07 ± 0.91 & 65.11 ± 1.05 & 65.40 & \textbf{5.2} \\
\bottomrule
\end{tabular}
\caption{Comparison of 5-way 1-shot performance on the last 5 unseen datasets of Meta-Dataset. These methods are trained on the first 8 datasets of Meta-Dataset.}
\label{tab:meta_dataset_unseen}
\end{table*}



\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llllll}
\toprule
\textbf{Method} & \textbf{CIFAR-10} & \textbf{CIFAR-100} & \textbf{Omniglot} & \textbf{Mini-ImageNet} & \textbf{Avg. Latency (ms)} \\
\midrule
\multicolumn{6}{l}{\textbf{Weight Generation}} \\
\rowcolor{gray!20} Head generation (ours) 
  & 62.07 ± 0.33 ($\downarrow$1.13) 
  & 51.73 ± 0.25 ($\downarrow$0.69)
  & 97.12 ± 0.23 ($\downarrow$0.72) 
  & 68.10 ± 0.24 ($\downarrow$0.82) 
  & 3.5 ($\downarrow$4.4) \\
Full generation 
  & 63.20 ± 0.36 
  & 52.42 ± 0.23 
  & 97.84 ± 0.25 
  & 68.92 ± 0.21 
  & 7.9 \\
\midrule
\multicolumn{6}{l}{\textbf{Gradient Descent Fine-Tuning}} \\
Head fine-tuning 
  & - & - 
  & 94.94 ± 0.27 ($\downarrow$0.45) 
  & 46.36 ± 0.28 ($\downarrow$0.71) 
  & 8.2 ($\downarrow$12.5) \\
Full fine-tuning 
  & - & - 
  & 95.39 ± 0.18 
  & 47.07 ± 0.26 
  & 20.7 \\
\bottomrule
\end{tabular}}
\caption{Comparison between head-only and full-network tuning. Arrows indicate the trade-off between accuracy and latency improvement.}
\label{tab:schedule_ablation}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llllll}
    \toprule
     && \multicolumn{2}{c}{\textbf{MRPC}} & \multicolumn{2}{c}{\textbf{QNLI}} \\
     \cmidrule(lr){3-4}
     \cmidrule(lr){5-6}
    \textbf{Fine-tuning Type} & \textbf{Method} & \textbf{Acc} & \textbf{Latency (h)} & \textbf{Acc} & \textbf{Latency (h)} \\
    \midrule
    Gradient-Based&Full-fine-tune (+Extra)   & 80.72 ± 0.62 ($\downarrow$ 9.52) & 1.47 ($\downarrow$ 0) & 80.91 ± 0.29 ($\downarrow$ 11.93) & 3.15 ($\downarrow$ 0) \\
    Gradient-Based&LoRA (+Extra)             & 83.91 ± 0.76 ($\downarrow$ 5.85) & 0.81 ($\downarrow$ 0) & 86.95 ± 0.21 ($\downarrow$ 6.37) & 1.76 ($\downarrow$ 0) \\
    Gradient-Based&AdaLoRA (+Extra)          & 82.64 ± 0.68 ($\downarrow$ 6.07) & 0.74 ($\downarrow$ 0) & 86.05 ± 0.28 ($\downarrow$ 7.12) & 1.68 ($\downarrow$ 0) \\
    Gradient-Based&DyLoRA (+Extra)           & 84.12 ± 0.87 ($\downarrow$ 5.47) & 0.76 ($\downarrow$ 0) & 85.52 ± 0.34 ($\downarrow$ 6.69) & 1.63 ($\downarrow$ 0) \\
    Gradient-Based&FourierFT (+Extra)        & 85.38 ± 0.58 ($\downarrow$ 4.65) & 0.68 ($\downarrow$ 0) & 85.95 ± 0.17 ($\downarrow$ 6.30) & 1.55 ($\downarrow$ 0) \\
    \midrule
    Gradient-Based&Full-fine-tune            & \textbf{90.24 ± 0.57} & 1.47 & 92.84 ± 0.26 & 3.15 \\
    Gradient-Based&LoRA                      & 89.76 ± 0.69 & 0.81 & \textbf{93.32 ± 0.20} & 1.76 \\
    Gradient-Based&AdaLoRA                   & 88.71 ± 0.73 & 0.74 & 93.17 ± 0.25 & 1.68 \\
    Gradient-Based&DyLoRA                    & 89.59 ± 0.81 & 0.76 & 92.21 ± 0.32 & 1.63 \\
    Gradient-Based&FourierFT                 & 90.03 ± 0.54 & 0.68 & 92.25 ± 0.15 & 1.55 \\
    \rowcolor{gray!20}Weights Generation&Lv-Di (+Extra) (ours)        & 88.15 ± 0.62 & 0.22 & 90.96 ± 0.18 & 0.48 \\
    \rowcolor{gray!20}Weights Generation&Lt-Di (+Extra) (ours)       & 89.03 ± 0.56 & \textbf{0.19} & 91.52 ± 0.22 & \textbf{0.41} \\
    \bottomrule
\end{tabular}}
\caption{Accuracy and fine-tuning latency comparison on GLUE-MRPC and GLUE-QNLI tasks for different fine-tuning algorithms. "+Extra" denotes using the extra five training tasks, \ie, SST-2, QQP, RTE, WNIL, and CoLA, for pre-training.}
\label{tab:performance_fine-tune_time_comparison}
\end{table*}












